Object-Centric Latent Action Learning

Leveraging vast amounts of unlabeled internet video data for embodied AI is currently bottlenecked by the lack of action labels and the presence of action-correlated visual distractors. Although recent latent action policy optimization (LAPO) has shown promise in inferring proxy action labels from visual observations, its performance degrades significantly when distractors are present. To address this limitation, we propose a novel object-centric latent action learning framework that centers on objects rather than pixels. We leverage self-supervised object-centric pretraining to disentangle the movement of the agent and distracting background dynamics. This allows LAPO to focus on task-relevant interactions, resulting in more robust proxy-action labels, enabling better imitation learning and efficient adaptation of the agent with just a few action-labeled trajectories. We evaluated our method in eight visually complex tasks across the Distracting Control Suite (DCS) and Distracting MetaWorld (DMW). Our results show that object-centric pretraining mitigates the negative effects of distractors by 50%, as measured by downstream task performance: average return (DCS) and success rate (DMW).

==> tab/eval-returns-aaai.tex <==
% \begin{table*}[t]
% \begin{center}
%     % \begin{tabular}{l|c|c|cc|cc}
%     \begin{tabular}{l|c|c|rlrl}
%     \toprule
%     \multicolumn{1}{c}{\bf Task} 
%         &\multicolumn{1}{c}{\textbf{LAPO} } 
%         &\multicolumn{1}{c}{\textbf{LAPO-vanilla}} 
%         &\multicolumn{2}{c}{\textbf{LAPO-masks}}
%         &\multicolumn{2}{c}{ \textbf{LAPO-slots}} 
%         % &\multicolumn{1}{c}{\textbf{LAPO-VANILLA}} 
%         % &\multicolumn{2}{c}{\textbf{LAPO-MASKS}} 
%         % &\multicolumn{2}{c}{ \textbf{LAPO-SLOTS}} 
%         \\
%     &baseline&upper-bound&ours&&ours
%         \\
%     \midrule

%     cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.76 {\scriptsize ± 0.04} & 0.41 {\scriptsize ± 0.03} & +32\% & 0.55 {\scriptsize ± 0.04} & +58\%\\
%     hopper-hop & 0.03 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.08 {\scriptsize ± 0.01} & +20\% & 0.15 {\scriptsize ± 0.02} & +50\% \\
%     walker-run & 0.04 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.06 {\scriptsize ± 0.01} & +6\% & 0.12 {\scriptsize ± 0.01} & +27\% \\
%     humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.04 {\scriptsize ± 0.02} & +47\% & 0.06 {\scriptsize ± 0.01} & +105\% \\
%     \midrule
%     % Mean DCS-hard & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & +26\% & 0.22 {\scriptsize ± 0.02} & +52\% \
%     \textbf{Mean DCS-Hard} & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & \textbf{+26\%} & 0.22 {\scriptsize ± 0.02} & \textbf{+52\%} \\
    
%     % cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.65 {\scriptsize ± 0.03} & 0.41 {\scriptsize ± 0.04} & 0.400037 & 0.55 {\scriptsize ± 0.04} & +74\% \\
%     % hopper-hop & 0.03 {\scriptsize ± 0.01} & 0.23 {\scriptsize ± 0.03} & 0.00 {\scriptsize ± 0.00} & -0.167532 & 0.15 {\scriptsize ± 0.02} & +59\% \\
%     % walker-run & 0.04 {\scriptsize ± 0.00} & 0.28 {\scriptsize ± 0.06} & 0.03 {\scriptsize ± 0.00} & -0.035514 & 0.12 {\scriptsize ± 0.01} & +32\% \\
%     % humanoid-walk & 0.02 {\scriptsize ± 0.00} & 0.05 {\scriptsize ± 0.01} & 0.03 {\scriptsize ± 0.03} & 0.401139 & 0.06 {\scriptsize ± 0.01} & +133\% \\
%     % \midrule
%     % Mean DCS & 0.08 {\scriptsize ± 0.01} & 0.30 {\scriptsize ± 0.03} & 0.12 {\scriptsize ± 0.02} & 0.150000 & 0.22 {\scriptsize ± 0.02} & +64\% \\
    
        
%     \midrule
%     cheetah-run & 0.34 {\scriptsize ± 0.06} & 0.76 {\scriptsize ± 0.04} & 0.54 {\scriptsize ± 0.09} & +48\% & 0.50 {\scriptsize ± 0.07} & +38\% \\
%     hopper-hop & 0.05 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.15 {\scriptsize ± 0.01} & +46\% & 0.19 {\scriptsize ± 0.02} & +64\% \\
%     walker-run & 0.10 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.21 {\scriptsize ± 0.05} & +52\% & 0.18 {\scriptsize ± 0.03} & +36\% \\
%     humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.05 {\scriptsize ± 0.02} & +67\% & 0.09 {\scriptsize ± 0.02} & +174\% \\
%     \midrule
%     % Mean DCS & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & +50\% & 0.24 {\scriptsize ± 0.03} & +50\% \\   
%     \textbf{Mean DCS} & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & \textbf{+50\%} & 0.24 {\scriptsize ± 0.03} & \textbf{+50\%} \\   
    
%     \midrule
%     hammer & 0.75 {\scriptsize ± 0.07} & 0.98 {\scriptsize ± 0.01} & 0.96 {\scriptsize ± 0.01} & +91\% & 0.99 {\scriptsize ± 0.02} & +102\% \\
%     bin-picking & 0.18 {\scriptsize ± 0.08} & 0.74 {\scriptsize ± 0.10} & 0.49 {\scriptsize ± 0.10} & +56\% & 0.33 {\scriptsize ± 0.08} & +27\% \\
%     basketball & 0.17 {\scriptsize ± 0.03} & 0.51 {\scriptsize ± 0.07} & 0.34 {\scriptsize ± 0.09} & +50\% & 0.37 {\scriptsize ± 0.09} & +58\% \\
%     soccer & 0.14 {\scriptsize ± 0.06} & 0.36 {\scriptsize ± 0.08} & 0.21 {\scriptsize ± 0.08} & +34\% & 0.23 {\scriptsize ± 0.06} & +41\% \\
%     \midrule
%     % Mean DMW & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & +55\% & 0.48 {\scriptsize ± 0.06} & +50\% \\ 
%     \textbf{Mean DMW} & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & \textbf{+55\%} & 0.48 {\scriptsize ± 0.06} & \textbf{+50\%} \\ 
%     \bottomrule
%     \end{tabular}
% \end{center}
% % \caption{Normalized evaluation returns for Distracting Control Suite(-Hard) tasks and normalized success rates for Distracting MetaWorld tasks of the BC agent trained on latent actions for different tasks. 
% % TL;DR:  LAPO's performance drops in the presence of distractors. Object-centric learning, using slots and masks, reduces this gap.
% % Each value represents the average score across different amounts of fine-tuning labeled trajectories and three random seeds. The BC agent trained with access to the full dataset of ground-truth actions would achieve a score of 1 for each task. 
% % The relative performance gain is given as 
% % $\small{\frac{\text{LAPO}\ -\ \text{LAPO-slots/masks}}{\text{LAPO}\ -\ \text{LAPO-vanilla}}}$.}
% \caption{
% \textbf{Object-centric pretraining significantly mitigates visual distractors.} 
% \textbf{DCS-Hard} extends the Distracting Control Suite with additional visual distractions: camera movement and color variation, in addition to dynamic background videos—making it substantially more challenging than standard DCS. 
% DMW includes dynamic backgrounds in manipulation tasks. 
% We report normalized evaluation returns (DCS variants) and success rates (DMW), where a score of 1.0 corresponds to a behavior cloning (BC) agent trained on the full set of ground-truth actions. 
% Each value averages performance across varying amounts of fine-tuning data and three random seeds.
% The relative performance gain is defined as:
% $
% \frac{\text{LAPO-slots/masks} - \text{LAPO}}{\text{LAPO-vanilla} - \text{LAPO}} \times 100\%
% $.
% This measures how much of the \emph{recoverable gap} (between distracted and clean data) is closed by our method. Our methods, \textbf{LAPO-slots} and \textbf{LAPO-masks}, achieve large gains over the distracted baseline (\textbf{LAPO}), closing up to \textbf{52--55\%} of the performance gap to the clean-data upper bound (\textbf{LAPO-vanilla}).
% }
% \label{table:eval-returns}
% \label{table:eval-returns}
% \end{table*}

%%%%%%%%%%%%%%%%%

% \begin{table*}[t]
% \begin{center}
% \begin{tabular}{l|c|c|rlrl}
% \toprule
% \multicolumn{1}{c}{\bf Task Description (Metric)} 
%     & \multicolumn{1}{c}{\textbf{LAPO}} 
%     & \multicolumn{1}{c}{\textbf{LAPO-vanilla}} 
%     & \multicolumn{2}{c}{\textbf{LAPO-masks}} 
%     & \multicolumn{2}{c}{\textbf{LAPO-slots}} \\
%     & baseline & upper-bound & \multicolumn{2}{c}{ours} & \multicolumn{2}{c}{ours} \\
% \midrule

% \multicolumn{7}{l}{\textbf{Distracting Control Suite-Hard (DCS-Hard)} \textit{(Normalized Return)}} \\
% \midrule
% cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.76 {\scriptsize ± 0.04} & 0.41 {\scriptsize ± 0.03} & +32\% & 0.55 {\scriptsize ± 0.04} & +58\% \\
% hopper-hop   & 0.03 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.08 {\scriptsize ± 0.01} & +20\% & 0.15 {\scriptsize ± 0.02} & +50\% \\
% walker-run   & 0.04 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.06 {\scriptsize ± 0.01} & +6\%  & 0.12 {\scriptsize ± 0.01} & +27\% \\
% humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.04 {\scriptsize ± 0.02} & +47\% & 0.06 {\scriptsize ± 0.01} & +105\% \\
% \textbf{MEAN} & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & \textbf{+26\%} & 0.22 {\scriptsize ± 0.02} & \textbf{+52\%} \\
% \midrule

% \multicolumn{7}{l}{\textbf{Distracting Control Suite (DCS)} \textit{(Normalized Return)}} \\
% \midrule
% cheetah-run  & 0.34 {\scriptsize ± 0.06} & 0.76 {\scriptsize ± 0.04} & 0.54 {\scriptsize ± 0.09} & +48\% & 0.50 {\scriptsize ± 0.07} & +38\% \\
% hopper-hop   & 0.05 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.15 {\scriptsize ± 0.01} & +46\% & 0.19 {\scriptsize ± 0.02} & +64\% \\
% walker-run   & 0.10 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.21 {\scriptsize ± 0.05} & +52\% & 0.18 {\scriptsize ± 0.03} & +36\% \\
% humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.05 {\scriptsize ± 0.02} & +67\% & 0.09 {\scriptsize ± 0.02} & +174\% \\
% \textbf{MEAN} & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & \textbf{+50\%} & 0.24 {\scriptsize ± 0.03} & \textbf{+50\%} \\
% \midrule

% \multicolumn{7}{l}{\textbf{Distracting MetaWorld (DMW)} \textit{(Normalized Success Rate)}} \\
% \midrule
% Hammer & 0.75 {\scriptsize ± 0.07} & 0.98 {\scriptsize ± 0.01} & 0.96 {\scriptsize ± 0.01} & +91\% & 0.99 {\scriptsize ± 0.02} & +102\% \\
% Bin-Picking & 0.18 {\scriptsize ± 0.08} & 0.74 {\scriptsize ± 0.10} & 0.49 {\scriptsize ± 0.10} & +56\% & 0.33 {\scriptsize ± 0.08} & +27\% \\
% Basketball & 0.17 {\scriptsize ± 0.03} & 0.51 {\scriptsize ± 0.07} & 0.34 {\scriptsize ± 0.09} & +50\% & 0.37 {\scriptsize ± 0.09} & +58\% \\
% Soccer & 0.14 {\scriptsize ± 0.06} & 0.36 {\scriptsize ± 0.08} & 0.21 {\scriptsize ± 0.08} & +34\% & 0.23 {\scriptsize ± 0.06} & +41\% \\
% \textbf{MEAN} & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & \textbf{+55\%} & 0.48 {\scriptsize ± 0.06} & \textbf{+50\%} \\
% \bottomrule
% \end{tabular}
% \end{center}

% \caption{
% }
% \label{table:eval-returns}
% \end{table*}


\begin{table*}[t]
\begin{center}
\begin{tabular}{c|l|c|c|rlrl}
\toprule
    \bf Environment \& 
    & \multicolumn{1}{|c|}{\bf Task \&}
    & \bf LAPO
    & \bf{LAPO-clean}
    & \multicolumn{2}{c}{\textbf{LAPO-masks}} 
    & \multicolumn{2}{c}{\textbf{LAPO-slots}} \\
    \bf Metric
    & \bf mean over tasks
    & baseline 
    & upper-bound 
    & \multicolumn{1}{|c}{ours} 
    & \multicolumn{1}{c}{+\textit{gain}\%} 
    & \multicolumn{1}{c}{ours} 
    & \multicolumn{1}{c}{+\textit{gain}\%} \\
\midrule

% \multirow{5}{*}{\shortstack[c]{\textbf{Distracting} \\ \textbf{Control Suite-Hard} \\ \textit{(Normalized Return)}}}
\multirow{5}{*}{\shortstack[c]{\textbf{DCS-Hard} \\ \textit{(Normalized Return)}}}
    & cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.76 {\scriptsize ± 0.04} & 0.41 {\scriptsize ± 0.03} & +32\% & 0.55 {\scriptsize ± 0.04} & +58\% \\
    & hopper-hop  & 0.03 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.08 {\scriptsize ± 0.01} & +20\% & 0.15 {\scriptsize ± 0.02} & +50\% \\
    & walker-run  & 0.04 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.06 {\scriptsize ± 0.01} & +6\%  & 0.12 {\scriptsize ± 0.01} & +27\% \\
    & humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.04 {\scriptsize ± 0.02} & +47\% & 0.06 {\scriptsize ± 0.01} & +105\% \\
\cmidrule(l){2-8}
    & \textbf{mean} & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & \textbf{+26\%} & 0.22 {\scriptsize ± 0.02} & \textbf{+52\%} \\
\midrule

% \multirow{5}{*}{\shortstack[c]{\textbf{Distracting} \\ \textbf{Control Suite} \\ \\ \textit{(Normalized Return)}}}
\multirow{5}{*}{\shortstack[c]{\textbf{DCS} \\ \\ \textit{(Normalized Return)}}}
    & cheetah-run & 0.34 {\scriptsize ± 0.06} & 0.76 {\scriptsize ± 0.04} & 0.54 {\scriptsize ± 0.09} & +48\% & 0.50 {\scriptsize ± 0.07} & +38\% \\
    & hopper-hop  & 0.05 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.15 {\scriptsize ± 0.01} & +46\% & 0.19 {\scriptsize ± 0.02} & +64\% \\
    & walker-run  & 0.10 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.21 {\scriptsize ± 0.05} & +52\% & 0.18 {\scriptsize ± 0.03} & +36\% \\
    & humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.05 {\scriptsize ± 0.02} & +67\% & 0.09 {\scriptsize ± 0.02} & +174\% \\
\cmidrule(l){2-8}
    & \textbf{mean} & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & \textbf{+50\%} & 0.24 {\scriptsize ± 0.03} & \textbf{+50\%} \\
\midrule

% \multirow{5}{*}{\shortstack[c]{\textbf{Distracting} \\ \textb?f{MetaWorld} \\ \textit{(Normalized Success Rate)}}}
\multirow{5}{*}{\shortstack[c]{\textbf{DMW} \\ \textit{(Normalized Success Rate)}}}
    & hammer & 0.75 {\scriptsize ± 0.07} & 0.98 {\scriptsize ± 0.01} & 0.96 {\scriptsize ± 0.01} & +91\% & 0.99 {\scriptsize ± 0.02} & +102\% \\
    & bin-picking & 0.18 {\scriptsize ± 0.08} & 0.74 {\scriptsize ± 0.10} & 0.49 {\scriptsize ± 0.10} & +56\% & 0.33 {\scriptsize ± 0.08} & +27\% \\
    & basketball & 0.17 {\scriptsize ± 0.03} & 0.51 {\scriptsize ± 0.07} & 0.34 {\scriptsize ± 0.09} & +50\% & 0.37 {\scriptsize ± 0.09} & +58\% \\
    & soccer & 0.14 {\scriptsize ± 0.06} & 0.36 {\scriptsize ± 0.08} & 0.21 {\scriptsize ± 0.08} & +34\% & 0.23 {\scriptsize ± 0.06} & +41\% \\
\cmidrule(l){2-8}
    & \textbf{mean} & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & \textbf{+55\%} & 0.48 {\scriptsize ± 0.06} & \textbf{+50\%} \\
\bottomrule
\end{tabular}
\end{center}

\caption{Object-centric pretraining substantially improves robustness to visual distractors, where standard imitation learning from observation methods like LAPO struggle. In environments with visual distractors: dynamic background videos (DCS and DMW) and additional camera motion and color variation (DCS-Hard), LAPO's performance is significantly degraded compared to the clean-data upper bound. We report normalized evaluation returns (DCS) and success rates (DMW) for a behavior cloning (BC) agent trained on latent actions, where a score of 1.0 corresponds to a BC agent trained on the full set of ground-truth actions. Each value averages performance across varying amounts of fine-tuning data and three random seeds. The relative performance gain is defined as:
$
\frac{\text{LAPO-slots/masks}\,\, -\,\,  \text{LAPO}}{\text{LAPO-clean}\,\, -\,\, \text{LAPO}} \times 100\%
$.
This measures the fraction of the recoverable performance gap between the distracted baseline (LAPO) and the clean-data performance (LAPO-clean) that our method recovers. LAPO-slots and LAPO-masks achieve large improvements over LAPO, closing up to $\sim 50\%$ of the gap, demonstrating that object-centric representations effectively mitigate the negative effects of visual distractions.}
\label{table:eval-returns}
\end{table*}

==> tab/eval-returns.tex <==
\begin{table}[t]
\caption{Normalized evaluation returns (DCS) and normalized success rates (DMW) of the BC agent trained on latent actions for different tasks. 
TL;DR:  LAPO's performance drops in the presence of distractors. Object-centric learning, using slots and masks, reduces this gap.
Each value represents the average score across different amounts of fine-tuning labeled trajectories and three random seeds. The BC agent trained with access to the full dataset of ground-truth actions would achieve a score of 1 for each task. 
The relative performance gain is given as 
$\small{\frac{\text{LAPO}\ -\ \text{LAPO-slots/masks}}{\text{LAPO}\ -\ \text{LAPO-vanilla}}}$.}
\label{table:eval-returns}
\begin{center}
    \adjustbox{max width=\textwidth}{
    % \begin{tabular}{l|c|c|cc|cc}
    \begin{tabular}{l|c|c|rlrl}
    \toprule
    \multicolumn{1}{c}{\bf Task} 
        &\multicolumn{1}{c}{\textbf{LAPO} } 
        &\multicolumn{1}{c}{\textbf{LAPO-vanilla}} 
        &\multicolumn{2}{c}{\textbf{LAPO-masks}} 
        &\multicolumn{2}{c}{ \textbf{LAPO-slots}} 
        % &\multicolumn{1}{c}{\textbf{LAPO-VANILLA}} 
        % &\multicolumn{2}{c}{\textbf{LAPO-MASKS}} 
        % &\multicolumn{2}{c}{ \textbf{LAPO-SLOTS}} 
        \\
    &baseline&upper-bound&ours&&ours
        \\
    \midrule

    cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.76 {\scriptsize ± 0.04} & 0.41 {\scriptsize ± 0.03} & +32\% & 0.55 {\scriptsize ± 0.04} & +58\%\\
    hopper-hop & 0.03 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.08 {\scriptsize ± 0.01} & +20\% & 0.15 {\scriptsize ± 0.02} & +50\% \\
    walker-run & 0.04 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.06 {\scriptsize ± 0.01} & +6\% & 0.12 {\scriptsize ± 0.01} & +27\% \\
    humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.04 {\scriptsize ± 0.02} & +47\% & 0.06 {\scriptsize ± 0.01} & +105\% \\
    \midrule
    % Mean DCS-hard & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & +26\% & 0.22 {\scriptsize ± 0.02} & +52\% \
    \textbf{Mean DCS-hard} & 0.08 {\scriptsize ± 0.01} & 0.35 {\scriptsize ± 0.04} & 0.15 {\scriptsize ± 0.02} & \textbf{+26\%} & 0.22 {\scriptsize ± 0.02} & \textbf{+52\%} \\
    
    % cheetah-run & 0.24 {\scriptsize ± 0.02} & 0.65 {\scriptsize ± 0.03} & 0.41 {\scriptsize ± 0.04} & 0.400037 & 0.55 {\scriptsize ± 0.04} & +74\% \\
    % hopper-hop & 0.03 {\scriptsize ± 0.01} & 0.23 {\scriptsize ± 0.03} & 0.00 {\scriptsize ± 0.00} & -0.167532 & 0.15 {\scriptsize ± 0.02} & +59\% \\
    % walker-run & 0.04 {\scriptsize ± 0.00} & 0.28 {\scriptsize ± 0.06} & 0.03 {\scriptsize ± 0.00} & -0.035514 & 0.12 {\scriptsize ± 0.01} & +32\% \\
    % humanoid-walk & 0.02 {\scriptsize ± 0.00} & 0.05 {\scriptsize ± 0.01} & 0.03 {\scriptsize ± 0.03} & 0.401139 & 0.06 {\scriptsize ± 0.01} & +133\% \\
    % \midrule
    % Mean DCS & 0.08 {\scriptsize ± 0.01} & 0.30 {\scriptsize ± 0.03} & 0.12 {\scriptsize ± 0.02} & 0.150000 & 0.22 {\scriptsize ± 0.02} & +64\% \\
    
        
    \midrule
    cheetah-run & 0.34 {\scriptsize ± 0.06} & 0.76 {\scriptsize ± 0.04} & 0.54 {\scriptsize ± 0.09} & +48\% & 0.50 {\scriptsize ± 0.07} & +38\% \\
    hopper-hop & 0.05 {\scriptsize ± 0.01} & 0.27 {\scriptsize ± 0.03} & 0.15 {\scriptsize ± 0.01} & +46\% & 0.19 {\scriptsize ± 0.02} & +64\% \\
    walker-run & 0.10 {\scriptsize ± 0.01} & 0.32 {\scriptsize ± 0.07} & 0.21 {\scriptsize ± 0.05} & +52\% & 0.18 {\scriptsize ± 0.03} & +36\% \\
    humanoid-walk & 0.02 {\scriptsize ± 0.01} & 0.06 {\scriptsize ± 0.01} & 0.05 {\scriptsize ± 0.02} & +67\% & 0.09 {\scriptsize ± 0.02} & +174\% \\
    \midrule
    % Mean DCS & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & +50\% & 0.24 {\scriptsize ± 0.03} & +50\% \\   
    \textbf{Mean DCS} & 0.13 {\scriptsize ± 0.02} & 0.35 {\scriptsize ± 0.04} & 0.24 {\scriptsize ± 0.04} & \textbf{+50\%} & 0.24 {\scriptsize ± 0.03} & \textbf{+50\%} \\   
    
    \midrule
    hammer & 0.75 {\scriptsize ± 0.07} & 0.98 {\scriptsize ± 0.01} & 0.96 {\scriptsize ± 0.01} & +91\% & 0.99 {\scriptsize ± 0.02} & +102\% \\
    bin-picking & 0.18 {\scriptsize ± 0.08} & 0.74 {\scriptsize ± 0.10} & 0.49 {\scriptsize ± 0.10} & +56\% & 0.33 {\scriptsize ± 0.08} & +27\% \\
    basketball & 0.17 {\scriptsize ± 0.03} & 0.51 {\scriptsize ± 0.07} & 0.34 {\scriptsize ± 0.09} & +50\% & 0.37 {\scriptsize ± 0.09} & +58\% \\
    soccer & 0.14 {\scriptsize ± 0.06} & 0.36 {\scriptsize ± 0.08} & 0.21 {\scriptsize ± 0.08} & +34\% & 0.23 {\scriptsize ± 0.06} & +41\% \\
    \midrule
    % Mean DMW & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & +55\% & 0.48 {\scriptsize ± 0.06} & +50\% \\ 
    \textbf{Mean DMW} & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & \textbf{+55\%} & 0.48 {\scriptsize ± 0.06} & \textbf{+50\%} \\ 
    \bottomrule
    \end{tabular}}
\end{center}
\vskip -0.1in
\end{table}

% \begin{table}[t]
% \caption{Normalized evaluation returns of the BC agent trained on latent actions for different tasks. 
% TL;DR:  LAPO's performance drops by x3.9 in the presence of distractors. Object-centric learning, using slots and masks, reduces this gap.
% % The rows represent corresponding tasks from the Distraction Control Suite (DSC), with the last row showing the average action probe MSE across all tasks. The columns represent the following approaches: \emph{lapo}: baseline latent action pretraining (LAPO) \citep{schmidt2024learningactactions} trained on the Distraction Control Suite (DCS); \emph{lapo-no-distractors}: LAPO trained on non-distracted observation data; \emph{lapo-slots} and \emph{lapo-masks}: models following the object-centric latent action pretraining pipeline described in \Cref{section:oc-lapo}. 
% Each value represents the average MSE across three different amounts of fine-tuning labeled trajectories and three random seeds. The values are scaled by 100, so the BC agent trained with access to the full dataset of ground-truth actions would achieve a score of 100 for each task.} %\textcolor{red}{change scores from mean to scores on 128 trajectories, use for this table formula $\frac{lapo - slots/masks}{lapo - vanilla}$}
% \label{table:eval-returns}
% \begin{center}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{l|r|rr|rr|rrrr}
%     \toprule
%     \multicolumn{1}{c}{\bf Task} 
%         &\multicolumn{1}{c}{\bf lapo} &\multicolumn{2}{c}{\bf lapo-masks (ours)} 
%         &\multicolumn{2}{c}{\bf lapo-slots (ours)} &\multicolumn{2}{c}{\bf lapo-no-distractors} \\
%     \midrule
%     % archive submission
%     cheetah-run & 23.0 $\pm$ 6.0 & 39.0 $\pm$ 1.0 & \colorbox{cyan!20}{x1.7} & 50 $\pm$ 1.0    & \colorbox{cyan!20}{x2.2} & 69.0 $\pm$ 14.0   & x3.1\\
%     walker-run & 4.0 $\pm$ 0.7 &  7.4 $\pm$ 2.8  & \colorbox{cyan!20}{x1.8} & 8.4 $\pm$ 3.0 & \colorbox{cyan!20}{x2.1} & 22.0 $\pm$ 19.0   & x5.5\\
%     hopper-hop & 3.2 $\pm$ 1.5 & 10.8 $\pm$ 0.6  & \colorbox{cyan!20}{x3.4} & 16 $\pm$ 3.0 & \colorbox{cyan!20}{x5.0} & 25.0 $\pm$ 9.0    & x7.7\\
%     humanoid-walk & 0.8 $\pm$ 0.4 & 5.9 $\pm$ 0.7& \colorbox{cyan!20}{x7.0} & 6.0 $\pm$ 0.2 & \colorbox{cyan!20}{x7.0} & 3.8 $\pm$ 3.1 & x4.5\\
%     \midrule
%     average & 7.7 & 16 & \colorbox{cyan!20}{x2.0} & 20 & \colorbox{cyan!20}{x2.6} & 30 & x3.9 \\
%     \midrule

%     % % archive submission + updated 'lapo-no-distractors'
%     % cheetah-run & 23.0 $\pm$ 6.0 & 39.0 $\pm$ 1.0 & \colorbox{cyan!20}{x1.7} & 50 $\pm$ 1.0 & \colorbox{cyan!20}{x2.2} & 76.3 $\pm$ 3.8   & x3.3\\
%     % walker-run & 4.0 $\pm$ 0.7 &  7.4 $\pm$ 2.8  & \colorbox{cyan!20}{x1.8} & 8.4 $\pm$ 3.0 & \colorbox{cyan!20}{x2.1} & 26.6 $\pm$ 3.0   & x6.7\\
%     % hopper-hop & 3.2 $\pm$ 1.5 & 10.8 $\pm$ 0.6  & \colorbox{cyan!20}{x3.4} & 16 $\pm$ 3.0  & \colorbox{cyan!20}{x5.0} & 32.1 $\pm$ 8.3   & x2.5\\
%     % humanoid-walk & 0.8 $\pm$ 0.4 & 5.9 $\pm$ 0.7& \colorbox{cyan!20}{x7.0} & 6.0 $\pm$ 0.2 & \colorbox{cyan!20}{x7.0} & 5.8  $\pm$ 0.8 & x7.2\\
%     % \midrule
%     % average & 7.7 & 16 & \colorbox{cyan!20}{x2.0} & 20 & \colorbox{cyan!20}{x2.6} & 35 & x4.5 \\
%     % \midrule

%     only background (mean over traj budjets)
%     cheetah-run & 34.0 $\pm$ 6.0 & 54.3 $\pm$ 9.3 & \colorbox{cyan!20}{x1.6} & 50.0 $\pm$ 6.7 & \colorbox{cyan!20}{x1.5} & 76.3 $\pm$ 4.0 & x2.4 \\
%     hopper-hop & 4.7 $\pm$ 1.4 & 14.9 $\pm$ 1.2 & \colorbox{cyan!20}{x3.4} & 18.7 $\pm$ 2.5 & \colorbox{cyan!20}{x4.1} & 26.6 $\pm$ 3.5 & x6.2 \\
%     walker-run & 9.6 $\pm$ 1.4 & 21.3 $\pm$ 5.0 & \colorbox{cyan!20}{x2.1} & 17.6 $\pm$ 2.5 & \colorbox{cyan!20}{x1.6} & 32.1 $\pm$ 6.6 & x3.1 \\
%     humanoid-walk & 2.0 $\pm$ 0.6 & 4.5 $\pm$ 1.6 & \colorbox{cyan!20}{x1.9} & 8.5 $\pm$ 1.6 & \colorbox{cyan!20}{x4.6} & 5.8 $\pm$ 1.4 & x2.8 \\
    
%     only background (128 traj budjets)
%     cheetah-run & 34.0 $\pm$ 5.3 & 54.3 $\pm$ 4.1 & \colorbox{cyan!20}{x1.6} & 50.0 $\pm$ 5.3 & \colorbox{cyan!20}{x1.5} & 76.3 $\pm$ 3.8 & x2.4 \\
%     hopper-hop & 4.7 $\pm$ 1.3 & 14.9 $\pm$ 2.6 & \colorbox{cyan!20}{x3.4} & 18.7 $\pm$ 3.0 & \colorbox{cyan!20}{x4.1} & 26.6 $\pm$ 3.0 & x6.2 \\
%     walker-run & 9.6 $\pm$ 1.0 & 21.3 $\pm$ 5.4 & \colorbox{cyan!20}{x2.1} & 17.6 $\pm$ 3.4 & \colorbox{cyan!20}{x1.6} & 32.1 $\pm$ 8.3 & x3.1 \\
%     humanoid-walk & 2.0 $\pm$ 1.1 & 4.5 $\pm$ 2.2 & \colorbox{cyan!20}{x1.9} & 8.5 $\pm$ 2.2 & \colorbox{cyan!20}{x4.6} & 5.8 $\pm$ 0.8 & x2.8 \\


%     \midrule

%     % average & 12.6 $\pm$ 2.4 & 23.8 $\pm$ 4.3 & \colorbox{cyan!20}{x2.3} & 23.7 $\pm$ 3.3 & \colorbox{cyan!20}{x3.0} &  35.2 $\pm$ 3.9 & x3.6 \\
%     % average & 12.6 & 23.8 & \colorbox{cyan!20}{x2.3} & 23.7 & \colorbox{cyan!20}{x3.0} &  35.2 & x3.6 \\
%     average & 12.6 & 23.8 & \colorbox{cyan!20}{x1.8} & 23.7 & \colorbox{cyan!20}{x1.8} &  35.2 & x2.8 \\
%     average & 13 & 24 & \colorbox{cyan!20}{x2} & 24 & \colorbox{cyan!20}{x2} &  35 & x3 \\


%     \toprule
%     & \textbf{LAPO} & \textbf{LAPO-VANILLA} & \textbf{LAPO-MASKS} (ours) & norm m & \textbf{LAPO-SLOTS} (ours) & norm s \\
%     \midrule
%     hammer & 0.75 {\scriptsize ± 0.07} & 0.98 {\scriptsize ± 0.01} & 0.96 {\scriptsize ± 0.01} & 0.906977 & 0.99 {\scriptsize ± 0.02} & 1.023256 \\
%     bin & 0.18 {\scriptsize ± 0.08} & 0.74 {\scriptsize ± 0.10} & 0.49 {\scriptsize ± 0.10} & 0.557143 & 0.33 {\scriptsize ± 0.08} & 0.271429 \\
%     basketball & 0.17 {\scriptsize ± 0.03} & 0.51 {\scriptsize ± 0.07} & 0.34 {\scriptsize ± 0.09} & 0.503817 & 0.37 {\scriptsize ± 0.09} & 0.583969 \\
%     soccer & 0.14 {\scriptsize ± 0.06} & 0.36 {\scriptsize ± 0.08} & 0.21 {\scriptsize ± 0.08} & 0.341176 & 0.23 {\scriptsize ± 0.06} & 0.411765 \\
%     Mean & 0.31 {\scriptsize ± 0.06} & 0.65 {\scriptsize ± 0.06} & 0.50 {\scriptsize ± 0.07} & 0.580000 & 0.48 {\scriptsize ± 0.06} & 0.570000 \\
%     \bottomrule
    

    
%     \bottomrule
%     \end{tabular}}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table}[t]
% \caption{Normalized evaluation returns of the BC agent trained on latent actions for different tasks. The rows represent corresponding tasks from the Distraction Control Suite (DSC), with the last row showing the average action probe MSE across all tasks. The columns represent the following approaches: 'lapo', which is the baseline latent action pretraining (LAPO) \citep{schmidt2024learningactactions} trained on the DCS; 'lapo-no-distractors', which is LAPO trained on non-distracted observation data; and 'lapo-slots' and 'lapo-masks', which are models following the object-centric latent action pretraining pipeline described in Section \ref{section:oc-lapo}. Each value represents the average MSE across three different amounts of fine-tuning labeled trajectories and three random seeds. The values are scaled by 100, so the BC agent trained with access to the full dataset of ground-truth actions would return a score of 100 for each task.}
% \label{table:eval-returns}
% \begin{center}
%     \adjustbox{max width=\textwidth}{
%     \begin{tabular}{l|r|rr|rr|rrrr}
%     \toprule
%     \multicolumn{1}{c}{\bf Task} 
%         &\multicolumn{1}{c}{\bf lapo} &\multicolumn{2}{c}{\bf lapo-masks (ours)} 
%         &\multicolumn{2}{c}{\bf lapo-slots (ours)} &\multicolumn{2}{c}{\bf lapo-no-distractors} \\
%     \midrule
%     cheetah-run & 23.0 $\pm$ 6.0 & 39.0 $\pm$ 1.0 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x1.7} & 50 $\pm$ 1.0    & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x2.2} & 69.0 $\pm$ 14.0   & \scalebox{0.8}{$\uparrow$} x3.1\\
%     walker-run & 4.0 $\pm$ 0.7 &  7.4 $\pm$ 2.8  & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x1.8} & 8.4 $\pm$ 3.0 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x2.1} & 22.0 $\pm$ 19.0   & \scalebox{0.8}{$\uparrow$} x5.5\\
%     hopper-hop & 3.2 $\pm$ 1.5 & 10.8 $\pm$ 0.6  & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x3.4} & 16 $\pm$ 3.0 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x5.0} & 25.0 $\pm$ 9.0    & \scalebox{0.8}{$\uparrow$} x7.7\\
%     humanoid-walk & 0.8 $\pm$ 0.4 & 5.9 $\pm$ 0.7& \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x7.0} & 6.0 $\pm$ 0.2 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x7.0} & 3.8 $\pm$ 3.1 & \scalebox{0.8}{$\uparrow$} x4.5\\
%     \midrule
%     average & 7.7 & 16 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x2.0} & 20 & \scalebox{0.8}{$\uparrow$} \colorbox{cyan!20}{x2.6} & 30 & \scalebox{0.8}{$\uparrow$} x3.9 \\
%     \bottomrule
%     \end{tabular}}
% \end{center}
% \end{table}

% \begin{table}[t]
% \caption{Eval returns. The corresponding BC agent return for each task would be 100.}
% \label{table:eval-returns}
% \begin{center}
%     \begin{tabular}{l|r|rr|rr|rrrr}
%     \toprule
%     \multicolumn{1}{c}{\bf Task} 
%         &\multicolumn{1}{c}{\bf lapo} &\multicolumn{2}{c}{\bf lapo-masks (ours)} 
%         &\multicolumn{2}{c}{\bf lapo-slots (ours)} &\multicolumn{2}{c}{\bf lapo-no-distractors} \\
%     \midrule
%     cheetah-run & 23.0 $\pm$ 6.0 & 39.0 $\pm$ 1.0  & x1.7 & 50.0 $\pm$ 1.0  & x2.2 & 69.0 $\pm$ 14.0   & x3.1\\
%     walker-run & 4.0 $\pm$ 0.7 &  7.4 $\pm$ 2.8  & x1.8 & 8.4 $\pm$ 3.0 & x2.1 & 22.0 $\pm$ 19.0   & x5.5\\
%     hopper-hop & 3.2 $\pm$ 1.5 & 10.8 $\pm$ 0.6  & x3.4 & 16.0 $\pm$ 3.0& x5.0 & 25.0 $\pm$ 9.0    & x7.7\\
%     humanoid-walk & 0.8 $\pm$ 0.4 & 5.9 $\pm$ 0.7& x7.0 & 6.0 $\pm$ 0.2 & x7.0 & 3.8 $\pm$ 3.1 & x4.5\\
%     \midrule
%     average & 7.7 $\pm$ 10.0 & 16.0 $\pm$ 16.0 & x3.5 & 20.0 $\pm$ 20.0 & x4.1 & 30.0 $\pm$ 28.0 & x5.2 \\
%     \bottomrule
%     \end{tabular}
% \end{center}
% \end{table}

==> tab/expert-bc-scores.tex <==
\begin{table}[h]
\caption{Comparison of the Performance of Algorithms. \emph{Expert} denotes  the policy used to collect the dataset trained on privileged information about minimal state of the observation (DCS) and expert policy from (DMW). \emph{BC-vanilla} denotes the scores of behavior cloning agents (BC) trained on full expert dataset to imitate expert policy on the privileged for our method true action labels and non-distracted observations. \emph{BC} denotes the scores of BC agents trained on full expert dataset to imitate expert policy on the distracted observations and privileged for our method true action labels.}
\label{table:expert-bc-scores}
\begin{center}
\begin{tabular}{l|c|c|c|c|c}
\toprule
\bf Task & \bf Expert policy & \bf Expert dataset & \bf BC-vanilla &\ \bf BC  &\ \bf Size, GB 
\\ 
\midrule
cheetah-run & 838 &  838 & 840 & 823 & 58\\
walker-run & 740 & 740 & 735 & 749 & 58\\
hopper-hop & 307 & 307 & 300 & 253 & 58\\
humanoid-walk & 617 & 617 & 601 & 428 & 59\\
\midrule
hammer & 1.0& 1.0 & 1.0 & 1.0 & 61\\
bin-picking & 1.0 & 1.0& 1.0 & 1.0 & 114\\
basketball & 0.96 & 1.0 & 1.0 & 1.0 & 87\\
soccer & 0.88 & 1.0& 1.0 & 0.8 & 67\\

\bottomrule
\end{tabular}
\end{center}
\end{table}


==> tab/latent-action-probes.tex <==
\begin{table}[t]
\caption{Mean action probes MSE for different tasks. 
TL;DR:  LAPO's performance drops by x5.3 in the presence of distractors. Object-centric learning, using slots and masks, reduces this gap, with notable improvements in tasks like cheetah-run and hopper-hop.
The rows represent corresponding tasks from the Distraction Control Suite (DSC), with the last row showing the average action probe MSE across all tasks. The columns represent the following approaches: \emph{lapo}: baseline latent action pretraining (LAPO) \citep{schmidt2024learningactactions} trained on the DCS; \emph{lapo-no-distractors}: LAPO trained on non-distracted observation data; \emph{lapo-slots} and \emph{lapo-masks}: models following the object-centric latent action pretraining pipeline described in \Cref{section:oc-lapo}. Each value represents the average MSE across 5 different latent action dimensions and 3 random seeds.
}
\label{table:mean-action-probe}
\begin{center}
% \setlength{\tabcolsep}{4pt}
\adjustbox{max width=\textwidth}{
\begin{tabular}{l|r|rr|rr|rrrr}
\toprule
\multicolumn{1}{c}{\bf Task} 
    &\multicolumn{1}{c}{\bf lapo} &\multicolumn{2}{c}{\bf lapo-masks (ours)} 
    &\multicolumn{2}{c}{\bf lapo-slots (ours)} &\multicolumn{2}{c}{\bf lapo-no-distractors} 
\\ 
\midrule
cheetah-run & 11.2 $\pm$ 6.9 &2.8 $\pm$ 1.0       & \colorbox{cyan!20}{x4.0}& 3.1 $\pm$ 0.9  &\colorbox{cyan!20}{x3.6} & 1.0 $\pm$ 0.6     & x12.0 \\
walker-run & 7.0 $\pm$ 3.2 &4.5 $\pm$ 1.7         & \colorbox{cyan!20}{x1.6} &5.3 $\pm$ 2.2   &\colorbox{cyan!20}{x1.3}  & 2.7 $\pm$ 1.3    & x2.6 \\ 
hopper-hop & 11.2 $\pm$ 4.9 & 3.5 $\pm$ 1.2       & \colorbox{cyan!20}{x3.2} &4.4 $\pm$ 1.8   &\colorbox{cyan!20}{x2.5}  & 1.9 $\pm$ 1.2    & x5.8 \\ 
humanoid-walk & 0.20 $\pm$ 0.04 & 0.18 $\pm$ 0.04 & \colorbox{cyan!20}{x1.1} &0.16 $\pm$ 0.04 &\colorbox{cyan!20}{x1.3}  &  0.13 $\pm$ 0.03 & x1.6 \\ 
\midrule
average & 7.4 & 2.7 & \colorbox{cyan!20}{x2.7} & 3.3 & \colorbox{cyan!20}{x2.5} & 1.4 & x5.3 \\
\bottomrule
\end{tabular}}
\end{center}
\vskip -0.1in
\end{table}

% \begin{table}[t]
% \caption{Mean action probes MSE for different tasks. The rows represent corresponding tasks from the Distraction Control Suite (DSC), with the last row showing the average action probe MSE across all tasks. The columns represent the following approaches: 'lapo': baseline latent action pretraining (LAPO) \citep{schmidt2024learningactactions} trained on the  DCS; 'lapo-no-distractors': LAPO trained on non-distracted observation data; 'lapo-slots' and 'lapo-masks': models following the object-centric latent action pretraining pipeline described in \Cref{section:oc-lapo}.
% Each value represents the average MSE across 5 different latent action dimensions and 3 random seeds.
% }
% \label{table:mean-action-probe}
% \begin{center}
% % \setlength{\tabcolsep}{4pt}
% \adjustbox{max width=\textwidth}{
% \begin{tabular}{l|r|rr|rr|rrrr}
% \toprule
% \multicolumn{1}{c}{\bf Task} 
%     &\multicolumn{1}{c}{\bf lapo} &\multicolumn{2}{c}{\bf lapo-masks (ours)} 
%     &\multicolumn{2}{c}{\bf lapo-slots (ours)} &\multicolumn{2}{c}{\bf lapo-no-distractors} 
% \\ 
% \midrule
% %            task_  masks-vs-lapo  slots-vs-lapo  no-distraction-vs-lapo
% % 0    cheetah-run       4.006120       3.590286               11.650915
% % 3     walker-run       1.569831       1.317752                2.581003
% % 1     hopper-hop       3.190084       2.517685                5.783559
% % 2  humanoid-walk       1.133421       1.264283                1.594804
% cheetah-run & 11.2 $\pm$ 6.9 &2.8 $\pm$ 1.0       & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x4.0}& 3.1 $\pm$ 0.9  &\scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x3.6} & 1.0 $\pm$ 0.6     &\scalebox{0.8}{$\downarrow$} x12.0 \\
% walker-run & 7.0 $\pm$ 3.2 &4.5 $\pm$ 1.7         & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x1.6} &5.3 $\pm$ 2.2   &\scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x1.3}  & 2.7 $\pm$ 1.3    &\scalebox{0.8}{$\downarrow$} x2.6 \\ 
% hopper-hop & 11.2 $\pm$ 4.9 & 3.5 $\pm$ 1.2       & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x3.2} &4.4 $\pm$ 1.8   &\scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x2.5}  & 1.9 $\pm$ 1.2    &\scalebox{0.8}{$\downarrow$} x5.8 \\ 
% humanoid-walk & 0.20 $\pm$ 0.04 & 0.18 $\pm$ 0.04 & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x1.1} &0.16 $\pm$ 0.04 &\scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x1.3}  &  0.13 $\pm$ 0.03 &\scalebox{0.8}{$\downarrow$} x1.6 \\ 
% \midrule
% average & 7.4 & 2.7 & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x2.7} & 3.3 & \scalebox{0.8}{$\downarrow$} \colorbox{cyan!20}{x2.5} & 1.4 & \scalebox{0.8}{$\downarrow$} x5.3 \\
% \bottomrule
% %       mean_orig_mean  mean_orig_std  mean_masks_mean  mean_masks_std  \
% % mean        7.402232       3.782005         2.740569        0.993732   
% % std         5.179797       2.910699         1.842492        0.702957   
% %       masks-vs-lapo  mean_slots_mean  mean_slots_std  slots-vs-lapo  \
% % mean       2.474864         3.265205        1.250060       2.172501   
% % std        1.350906         2.262229        0.981822       1.108260   
% %       mean_vanilla_mean  mean_vanilla_std  no-distraction-vs-lapo  
% % mean           1.437362          0.766513                5.402570  
% % std            1.133342          0.587233                4.533111 
% % cheetah-run & 11.2 $\pm$ 6.9 &2.8 $\pm$ 1.0 &       +82\%& 3.1 $\pm$ 0.9 &    +79\% & 1.0 $\pm$ 0.6  \\
% % walker-run & 7.0 $\pm$ 3.2   &4.5 $\pm$ 1.7 &       +59\% &5.3 $\pm$ 2.2 &    +39\% & 2.7 $\pm$ 1.3 \\ 
% % hopper-hop & 11.2 $\pm$ 4.9  & 3.5 $\pm$ 1.2 &      +83\% &4.4 $\pm$ 1.8 &    +73\% & 1.9 $\pm$ 1.2  \\ 
% % humanoid-walk & 0.20 $\pm$ 0.04 & 0.18 $\pm$ 0.04 & +32\%&  0.16 $\pm$ 0.04 & +56\%&  0.13 $\pm$ 0.03 \\ 
% \end{tabular}}
% \end{center}
% \end{table}

==> tab/parameters.tex <==
\begin{table}[h!]
\caption{Amount of parameters for different models. The rows represent the following approaches:
\emph{ocp}: denotes the number of parameters of the object-centric model;
\emph{lapo-slots}: denotes the number of parameters for latent action learning from vector representations; utilizing object-centric representations from a precollected dataset;
\emph{lapo}: denotes the number of parameters for latent action learning from images;
\emph{lapo-masks}: denotes the number of parameters for latent action learning from images, utilizing object-centric masks from a precollected dataset (using the same model as \emph{lapo});
\emph{bc}: Denotes the number of parameters of the behavior cloning agent trained on latent actions.
}
\label{table:training-duration}
\begin{center}
\begin{tabular}{l|r|r}
\toprule
\bf Method & \bf DCS& \bf DMW
\\ 
\midrule
ocp (total) & 92,149,776& 92,149,776  \\
ocp (trainable)&  6,343,440 &  6,343,440 \\
\midrule
lapo-slots & 89,186,432 & 15,491,776\\
lapo-masks & 211,847,849& 36,269,129\\
lapo & 211,847,849  & 36,269,129\\
\midrule
bc & 107,541,504 & 126,703,872\\
\bottomrule
\end{tabular}
\end{center}
\end{table}

% 15,491,776
% 227,276,800



==> tab/training-duration.tex <==
\begin{table}[h!]
\caption{Average training duration of the methods. The row represent the following approaches: \emph{ocp} denotes the time spent on object-centric pretraining stage which is common for both slots and masks; \emph{lapo-masks} and \emph{lapo-slots} denote the time spent on training latent action model, reading object-centric representations from a precollected dataset; \emph{lapo} denote the time spent on training latent action model, \emph{ocp + lapo-masks} and \emph{ocp + lapo-slots} denote the time for full pipeline of object-centric latent action learning}
\label{table:training-duration}
\begin{center}
\begin{tabular}{l|r|r}
\toprule
\bf Method & \bf Training Duration DCS & \bf Training Duration DMW\\ 
\midrule
ocp        & $\sim$ 6 h 30 m  & $\sim$ 8 h 30 m  \\
lapo-slots & $\sim$ 2 h 30 m& $\sim$ 1 h 30 m  \\
lapo-masks & $\sim$ 7 h 30 m& $\sim$ 2 h 30 m  \\
\midrule
lapo             & $\sim$ 7 h 30 m & $\sim$ 2 h 30 m \\
ocp + lapo-slots & $\sim$ 9 h 0 m  & $\sim$ 10 h 0 m \\
ocp + lapo-masks & $\sim$ 14 h 0 m& $\sim$ 11 h 00 m \\
\midrule
bc + finetuning & $\sim$ 3 h 2 m & $\sim$ 1 h 30 m \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

